Completeness results for quasi-categories of algebras, homotopy limits, and related general constructions

Consider a diagram of quasi-categories that admit and functors that preserve limits or colimits of a fixed shape. We show that any weighted limit whose weight is a projective cofibrant simplicial functor is again a quasi-category admitting these (co)limits and that they are preserved by the functors in the limit cone. In particular, the Bousfield-Kan homotopy limit of a diagram of quasi-categories admit any limits or colimits existing in and preserved by the functors in that diagram. In previous work, we demonstrated that the quasi-category of algebras for a homotopy coherent monad could be described as a weighted limit with projective cofibrant weight, so these results immediately provide us with important (co)completeness results for quasi-categories of algebras. These generalise most of the classical categorical results, except for a well known theorem which shows that limits lift to the category of algebras for any monad, regardless of whether its functor part preserves those limits. The second half of this paper establishes this more general result in the quasi-categorical setting: showing that the monadic forgetful functor of the quasi-category of algebras for a homotopy coherent monad creates all limits that exist in the base quasi-category, without further assumption on the monad. This proof relies upon a more delicate and explicit analysis of the particular weight used to define quasi-categories of algebras.

==> reedy_lab.tex <==
\newlabel{reedy:eq:reedy's.po}{{1.1}{2}{Introduction}{equation.1.1}{}}
\newlabel{reedy:eq:reedy's.delta}{{1.2}{3}{Introduction}{equation.1.2}{}}
\newlabel{reedy:ntn:index-stuff}{{1.4}{4}{general index notation}{thm.1.4}{}}
\newlabel{reedy:ex:tensor-cotensor}{{1.6}{5}{tensors and cotensors}{thm.1.6}{}}
\newlabel{reedy:defn:ends-and-coends}{{1.7}{6}{ends and coends}{thm.1.7}{}}
\newlabel{reedy:defn:cat-of-elts}{{1.8}{6}{categories of elements}{thm.1.8}{}}
\newlabel{reedy:obs:coend-in-sets}{{1.9}{7}{coends in sets}{thm.1.9}{}}
\newlabel{reedy:eq:pb-coends-in-sets}{{1.10}{7}{coends in sets}{equation.1.10}{}}
\newlabel{reedy:eq:wlimformula}{{1.12}{7}{weighted limits and colimits}{equation.1.12}{}}
\newlabel{reedy:ex:weighted-conical}{{1.13}{7}{terminal weights}{thm.1.13}{}}
\newlabel{reedy:ex:weighted-yoneda}{{1.14}{8}{representable weights}{thm.1.14}{}}
\newlabel{reedy:eq:yoneda}{{1.15}{8}{representable weights}{equation.1.15}{}}
\newlabel{reedy:ex:matching.preview}{{1.17}{8}{}{thm.1.17}{}}
\newlabel{reedy:obs:weighted.as.ordinary}{{1.19}{8}{weighted limits as ordinary limits}{thm.1.19}{}}
\newlabel{reedy:obs:wcolim-in-sets}{{1.21}{8}{weighted colimits in sets}{thm.1.21}{}}
\newlabel{reedy:sec:reedy}{{2}{9}{Reedy categories}{section.2}{}}
\newlabel{reedy:defn:reedy}{{2.1}{9}{Reedy categories}{thm.2.1}{}}
\newlabel{reedy:ex:poset.reedy}{{2.3}{9}{finite posets}{thm.2.3}{}}
\newlabel{reedy:ex:pushout.reedy.alt}{{2.4}{9}{the pushout diagram}{thm.2.4}{}}
\newlabel{reedy:ex:parallel.pair.reedy}{{2.5}{10}{the parallel pair}{thm.2.5}{}}
\newlabel{reedy:defn:factorisations}{{2.8}{10}{categories of factorisations}{thm.2.8}{}}
\newlabel{reedy:lem:reedy-fact-connect}{{2.9}{10}{}{thm.2.9}{}}
\newlabel{reedy:sec:latching}{{3}{11}{Latching and matching objects}{section.3}{}}
\newlabel{reedy:rec:skel-coskel}{{3.1}{11}{skeleta and coskeleta}{thm.3.1}{}}
\newlabel{reedy:eq:4}{{3.2}{12}{skeleta and coskeleta}{equation.3.2}{}}
\newlabel{reedy:obs:skel-colim}{{3.3}{12}{}{thm.3.3}{}}
\newlabel{reedy:eq:5}{{3.4}{12}{}{equation.3.4}{}}
\newlabel{reedy:lem:skeleta-colimit}{{3.5}{13}{}{thm.3.5}{}}
\newlabel{reedy:eq:6}{{3.6}{13}{}{equation.3.6}{}}
\newlabel{reedy:obs:skel-reps}{{3.7}{13}{skeleta of representables and factorisations}{thm.3.7}{}}
\newlabel{reedy:eq:sk-rep-coend}{{3.8}{13}{skeleta of representables and factorisations}{equation.3.8}{}}
\newlabel{reedy:lem:inductive.defn}{{3.10}{15}{inductive definition of diagrams}{thm.3.10}{}}
\newlabel{reedy:obs:inductive.defn}{{3.11}{15}{inductive definition of natural transformations}{thm.3.11}{}}
\newlabel{reedy:ex:sequence-induction}{{3.12}{15}{}{thm.3.12}{}}
\newlabel{reedy:defn:latching}{{3.13}{16}{latching and matching objects}{thm.3.13}{}}
\newlabel{reedy:ex:simp-latching-1}{{3.14}{16}{}{thm.3.14}{}}
\newlabel{reedy:obs:weights-latching}{{3.15}{16}{weights for latching and matching objects}{thm.3.15}{}}
\newlabel{reedy:eq:7}{{3.16}{16}{weights for latching and matching objects}{equation.3.16}{}}
\newlabel{reedy:lem:sk-rep-reedy}{{3.17}{17}{skeleta of the representables of a Reedy category}{thm.3.17}{}}
\newlabel{reedy:obs:cons-skeleta}{{3.18}{17}{characterising the boundary of a representable}{thm.3.18}{}}
\newlabel{reedy:ex:sequence.latching}{{3.19}{17}{}{thm.3.19}{}}
\newlabel{reedy:ex:pushout.latching}{{3.20}{17}{}{thm.3.20}{}}
\newlabel{reedy:ex:parallel.pair.latching}{{3.21}{18}{}{thm.3.21}{}}
\newlabel{reedy:ex:simp-latching-2}{{3.22}{18}{}{thm.3.22}{}}
\newlabel{reedy:obs:latching.ordinary.colimit}{{3.23}{18}{latching objects as ordinary colimits}{thm.3.23}{}}
\newlabel{reedy:sec:Leibniz-Reedy}{{4}{19}{Leibniz constructions and the Reedy model structure}{section.4}{}}
\newlabel{reedy:obs:box-product}{{4.2}{19}{Leibniz's formula}{thm.4.2}{}}
\newlabel{reedy:defn:leibniz}{{4.4}{20}{the Leibniz construction}{thm.4.4}{}}
\newlabel{reedy:eq:13}{{4.5}{20}{the Leibniz construction}{equation.4.5}{}}
\newlabel{reedy:ex:boundary-prod}{{4.6}{20}{}{thm.4.6}{}}
\newlabel{reedy:obs:leibniz-isos}{{4.7}{20}{Leibniz and structural isomorphisms}{thm.4.7}{}}
\newlabel{reedy:lem:leibniz-cocts}{{4.8}{21}{Leibniz and colimit preservation}{thm.4.8}{}}
\newlabel{reedy:eq:2varadj}{{4.9}{21}{\S \ Leibniz constructions}{equation.4.9}{}}
\newlabel{reedy:lem:leibniz-close}{{4.10}{21}{Leibniz and closures}{thm.4.10}{}}
\newlabel{reedy:obs:leibniz-lifting-properties}{{4.11}{22}{Leibniz and lifting properties}{thm.4.11}{}}
\newlabel{reedy:defn:relative-maps}{{4.14}{22}{relative latching and matching maps}{thm.4.14}{}}
\newlabel{reedy:obs:relative.lifting}{{4.16}{23}{relative latching and matching maps and lifting problems}{thm.4.16}{}}
\newlabel{reedy:eq:i-lift-p}{{4.17}{23}{relative latching and matching maps and lifting problems}{equation.4.17}{}}
\newlabel{reedy:thm:model-structure}{{4.18}{24}{the Reedy model structure}{thm.4.18}{}}
\newlabel{reedy:sec:Leibniz-rel-cell-cx}{{5}{24}{Leibniz constructions and cell complexes}{section.5}{}}
\newlabel{reedy:obs:leibniz-comp}{{5.1}{24}{Leibniz and composites}{thm.5.1}{}}
\newlabel{reedy:defn:transfinite-composites}{{5.3}{25}{transfinite composites}{thm.5.3}{}}
\newlabel{reedy:def:rel-cell}{{5.4}{25}{cell complexes}{thm.5.4}{}}
\newlabel{reedy:eq:10}{{5.5}{26}{cell complexes}{equation.5.5}{}}
\newlabel{reedy:ntn:phi-map}{{5.6}{26}{}{thm.5.6}{}}
\newlabel{reedy:lem:leibniz-tcofp}{{5.7}{26}{Leibniz bifunctors and cell complexes}{thm.5.7}{}}
\newlabel{reedy:eq:11}{{5.8}{27}{Leibniz constructions and cell complexes}{equation.5.8}{}}
\newlabel{reedy:obs:leibniz-tcofp}{{5.9}{27}{}{thm.5.9}{}}
\newlabel{reedy:ex:latch-comp}{{5.10}{28}{relative latching maps of composites II}{thm.5.10}{}}
\newlabel{reedy:cor:leibniz-tcofp}{{5.11}{28}{}{thm.5.11}{}}
\newlabel{reedy:prop:leibniz-tcofp}{{5.12}{28}{}{thm.5.12}{}}
\newlabel{reedy:sec:cellular}{{6}{29}{Cellular presentations and Reedy categories}{section.6}{}}
\newlabel{reedy:obs:two-sided}{{6.1}{29}{skeleta of two-sided representables}{thm.6.1}{}}
\newlabel{reedy:obs:building-skeleta-rep}{{6.2}{29}{building up for skeleta of representables}{thm.6.2}{}}
\newlabel{reedy:prop:building-up}{{6.3}{30}{general building up}{thm.6.3}{}}
\newlabel{reedy:eq:skel-seq}{{6.4}{31}{general building up}{equation.6.4}{}}
\newlabel{reedy:eq:c-cell}{{6.5}{31}{general building up}{equation.6.5}{}}
\newlabel{reedy:eq:skel-seq-cells}{{6.6}{31}{Cellular presentations and Reedy categories}{equation.6.6}{}}
\newlabel{reedy:cor:building-up}{{6.7}{32}{}{thm.6.7}{}}
\newlabel{reedy:cor:B-cell-complex}{{6.8}{32}{}{thm.6.8}{}}
\newlabel{reedy:ex:EZ.simp.set}{{6.9}{33}{}{thm.6.9}{}}
\newlabel{reedy:sec:proof}{{7}{33}{Proof of the Reedy model structure}{section.7}{}}
\newlabel{reedy:lem:triv-cof-char}{{7.1}{33}{}{thm.7.1}{}}
\newlabel{reedy:lem:lifting}{{7.3}{34}{lifting}{thm.7.3}{}}
\newlabel{reedy:lem:factorisation}{{7.4}{34}{factorisation}{thm.7.4}{}}
\newlabel{reedy:eq:factorisation-defn}{{7.5}{35}{Proof of the Reedy model structure}{equation.7.5}{}}
\newlabel{reedy:prop:reedy.cof.gen}{{7.7}{35}{}{thm.7.7}{}}
\newlabel{reedy:sec:hocolim}{{8}{36}{Homotopy limits and colimits}{section.8}{}}
\newlabel{reedy:ex:hocoeq}{{8.2}{37}{homotopy coequalisers}{thm.8.2}{}}
\newlabel{reedy:ex:hoeq}{{8.3}{37}{homotopy equalisers}{thm.8.3}{}}
\newlabel{reedy:prop:reedy.model.dual}{{8.4}{38}{}{thm.8.4}{}}
\newlabel{reedy:ex:mapping}{{8.5}{38}{mapping telescopes}{thm.8.5}{}}
\newlabel{reedy:eq:sequence}{{8.6}{38}{mapping telescopes}{equation.8.6}{}}
\newlabel{reedy:eq:sequence.replacement}{{8.7}{38}{mapping telescopes}{equation.8.7}{}}
\newlabel{reedy:ex:hopushout}{{8.8}{38}{homotopy pushouts}{thm.8.8}{}}
\newlabel{reedy:eq:pushout.compare}{{8.9}{39}{homotopy pushouts}{equation.8.9}{}}
\newlabel{reedy:ex:stupid-simplicial}{{8.10}{39}{}{thm.8.10}{}}
\newlabel{reedy:sec:connected-weights}{{9}{39}{Connected weights}{section.9}{}}
\newlabel{reedy:prop:2/3-SM7}{{9.1}{39}{}{thm.9.1}{}}
\newlabel{reedy:obs:fibrant.constants}{{9.2}{40}{}{thm.9.2}{}}
\newlabel{reedy:cor:connected.weights}{{9.4}{40}{}{thm.9.4}{}}
\newlabel{reedy:sec:simplicial}{{10}{41}{Simplicial model categories and geometric realization}{section.10}{}}
\newlabel{reedy:thm:simp.model.cat}{{10.3}{42}{}{thm.10.3}{}}
\newlabel{reedy:eq:simpmodelreedy}{{10.4}{42}{Simplicial model categories and geometric realization}{equation.10.4}{}}
\newlabel{reedy:obs:geo-filt}{{10.7}{43}{skeletal filtration of geometric realization}{thm.10.7}{}}
\newlabel{reedy:eq:reedy's.po2}{{10.8}{43}{skeletal filtration of geometric realization}{equation.10.8}{}}
\newlabel{reedy:tocindent-1}{0pt}
\newlabel{reedy:tocindent0}{15.59619pt}
\newlabel{reedy:tocindent1}{27.59326pt}
\newlabel{reedy:tocindent2}{0pt}
\newlabel{reedy:tocindent3}{0pt}

